Making Hybrid Languages: A Recipe

The dominant programming languages support only linear text to express ideas. Visual languages offer graphical representations for entire programs, when viewed with special tools. Hybrid languages, with support from existing tools, allow developers to express their ideas with a mix of textual and graphical syntax tailored to an application domain. This mix puts both kinds of syntax on equal footing and, importantly, the enriched language does not disrupt a programmer's typical workflow. This paper presents a recipe for equipping existing textual programming languages as well as accompanying IDEs with a mechanism for creating and using graphical interactive syntax. It also presents the first hybrid language and IDE created using the recipe.

==> Makefile <==
OPEN=open

.ONESHELL:

all: paper.pdf

venv: .env/touchfile

utils/node_modules: utils/package-lock.json
	(cd utils; npm ci)

.env/touchfile: deps/info.rkt
	raco pkg-env --clear .env
	touch .env/touchfile
	. .env/activate.sh
	raco pkg install --auto deps/

paper.tex: *.scrbl utils/node_modules venv
	. .env/activate.sh
	racket paper.scrbl > paper.tex

paper.pdf: *.scrbl utils/node_modules Images/how-interactive-syntax-works.pdf venv
	. .env/activate.sh
	racket paper.scrbl > paper.tex
	xelatex -interaction=nonstopmode paper.tex
	bibtex paper
	xelatex -interaction=nonstopmode paper.tex
	xelatex -interaction=nonstopmode paper.tex

draft: *.scrbl utils/node_modules Images/how-interactive-syntax-works.pdf venv
	. .env/activate.sh
	racket paper.scrbl -d > paper.tex
	xelatex -interaction=nonstopmode paper.tex
	bibtex paper
	xelatex -interaction=nonstopmode paper.tex
	xelatex -interaction=nonstopmode paper.tex


Images/how-interactive-syntax-works.pdf: Images/how-interactive-syntax-works.rkt
	raco test Images/how-interactive-syntax-works.rkt

leif: paper.pdf 
	cp paper.pdf argh.pdf 

fast: *.scrbl utils/node_modules venv
	. .env/activate.sh 
	racket paper.scrbl > paper.tex 
	xelatex -interaction=nonstopmode paper.tex && \
	echo "hopefully you're on macOS" 
	${OPEN} paper.pdf 

clean:
	rm -r prebuilt
	rm paper.pdf
	rm paper.aux
	rm paper.bbl
	rm paper.log
	rm paper.log
	rm paper.out

